What's in a Name? Answer Equivalence For Open-Domain Question Answering

A flaw in QA evaluation is that annotations often only provide one gold answer. Thus, model predictions semantically equivalent to the answer but superficially different are considered incorrect. This work explores mining alias entities from knowledge bases and using them as additional gold answers (i.e., equivalent answers). We incorporate answers for two settings: evaluation with additional answers and model training with equivalent answers. We analyse three QA benchmarks: Natural Questions, TriviaQA, and SQuAD. Answer expansion increases the exact match score on all datasets for evaluation, while incorporating it helps model training over real-world datasets. We ensure the additional answers are valid through a human post hoc evaluation.

==> 2021_emnlp_answer_equiv/sections/30-experiment.tex <==
\section{Experiment}
\label{sec:experiment}

% MOVED TO APPENDIX

\begin{table}[t]
  \jbgcomment{Perhaps give the average number of answers per question as well?}
\small
\center
\begin{tabular}{l|ccc}
\toprule
Dataset & Train & Dev & Test  \\
 \midrule
 NQ & 79168 & 8757 & 3610 \\
 TriviaQA & 78859 & 8763 & 11313 \\
SQuAD & 78840 & 8759 & 10570 \\
 \bottomrule
\end{tabular}
\caption{Number of questions in each dataset.}
\label{tab:statistics}
\end{table}


\subsection{Datasets}

Our experiments on \abr{nq}, \triviaqa{} and \squad{} study the effect of augmented evaluation and training. 
Since the official test sets are not released, we use the original dev set as the test set, and randomly split 10\% training data as the dev set. 
We briefly introduce each dataset and present the dataset statistics in Table~\ref{tab:statistics}. 
All of these datasets are extractive \abr{qa} datasets where answers are spans in Wikipedia articles. 

\paragraph{NQ} consists of information-seeking questions from Google search queries. We only consider short answers, which are answer spans in Wikipedia articles.

\paragraph{TriviaQA} consists of trivia questions with answers scraped from the Web.

\paragraph{SQuAD} (v1.1) was constructed as a reading comprehension benchmark. Its questions are written by annotators based on given paragraphs. We follow previous \abr{ODQA} works and use it in an open-domain setting. Speficially, we only use its questions and answers, without the corresponding passages associated with each question. Instead, we use \abr{dpr} to retrieve relevant passages for each question. 



\subsection{Setup}

For all experiments, we use \bert{}-base-uncased as the reader model. We train the model for four epochs, with batch size eight, and a learning rate of $3e-5$. We select the best checkpoint based on the \abr{em} score on the dev set and then evaluate the checkpoint on the test set.
%
We do not tune any dataset-specific hyper-parameters, use the same set of hyper-parameters for all of our experiments, and report \abr{em} scores on the test set for comparison.
%
Experiments are done on four 2080Ti \abr{gpu}s.



